Long-Short Transformer: Efficient Transformers for Language and Vision

Transformers have achieved success in both language and vision domains. However, it is prohibitively expensive to scale them to long sequences such as long documents or high-resolution images, because self-attention mechanism has quadratic time and memory complexities with respect to the input sequence length. In this paper, we propose Long-Short Transformer (Transformer-LS), an efficient self-attention mechanism for modeling long sequences with linear complexity for both language and vision tasks. It aggregates a novel long-range attention with dynamic projection to model distant correlations and a short-term attention to capture fine-grained local correlations. We propose a dual normalization strategy to account for the scale mismatch between the two attention mechanisms. Transformer-LS can be applied to both autoregressive and bidirectional models without additional complexity. Our method outperforms the state-of-the-art models on multiple tasks in language and vision domains, including the Long Range Arena benchmark, autoregressive language modeling, and ImageNet classification. For instance, Transformer-LS achieves 0.97 test BPC on enwik8 using half the number of parameters than previous method, while being faster and is able to handle 3x as long sequences compared to its full-attention version on the same hardware. On ImageNet, it can obtain the state-of-the-art results (e.g., a moderate size of 55.8M model solely trained on 224x224 ImageNet-1K can obtain Top-1 accuracy 84.1%), while being more scalable on high-resolution images. The source code and models are released at https://github.com/NVIDIA/transformer-ls .

==> Long-Short Transformer - NeurIPS 2021/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{dsfont}

\usepackage{amsthm}

\newcommand{\indicator}{{\mathds{1} }}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

%%% THEOREM etc.
\newtheorem{lemma}{Lemma}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{proposition}[lemma]{Proposition}

\theoremstyle{definition}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vsigma{{\bm{\sigma}}}
\def\vgamma{{\bm{\gamma}}}
\def\vbeta{{\bm{\beta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\text{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\cls}{{\sc Awt}}
\newcommand{\none}{{\sc None}}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Long-Short Transformer - NeurIPS 2021/sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work? 
    \answerYes{} We mentioned that as our future work in the conclusion section.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} Yes, we have included an investigation into the robustness of our vision models in the experiments. Also see Broader Impacts Section in Appendix.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Long-Short Transformer - NeurIPS 2021/sections/experiments.tex <==

\vspace{-.2em}
\section{Experiments}
\label{sec:experiments}
\vspace{-.2em}
%
In this section, we demonstrate the effectiveness and efficiency of our method in both language and vision domains. 
%
We use PyTorch for implementation and count the FLOPs using fvcore~\citep{fvcore}.



% Begin of LRA experiments  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bidirectional Modeling on Long Range Arena and IMDb}

%Begin Table %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
% \setlength{\columnsep}{25pt}%
% \setlength{\tabcolsep}{2pt}
\centering
\caption{\footnotesize 
Accuracy (\%) and FLOPs (G) on Long Range Arena (LRA), with the  model configs annotated (see Table~\ref{tbl:lra_configs} for more). All results are averages of 4 runs with different random seeds.}
\vspace{-.3em}
\label{tbl:lra}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcc|cc|cc|c}
\toprule
Task   & \multicolumn{2}{c}{ListOps}     & \multicolumn{2}{c}{Text}     & \multicolumn{2}{c}{Retrieval}             &   Average           \\
(mean $\pm$ std.) of sequence length   & \multicolumn{2}{c}{(888 $\pm$ 339)}     & \multicolumn{2}{c}{(1296 $\pm$ 893)}      & \multicolumn{2}{c}{(3987 $\pm$ 560)}  &    \\
\midrule
Model                      & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c}{FLOPs} & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c}{FLOPs} & \multicolumn{1}{c}{Acc. } & \multicolumn{1}{c}{FLOPs} & Acc. \\
\midrule
Full Attention~\citep{vaswani2017attention}          & 37.13                         & 1.21                          & 65.35                         & 4.57                          & \textbf{82.30}                         & 9.14         &       61.59          \\
% \midrule
Reformer~\citep{kitaev2020reformer} (2)              & 36.44                         & 0.27                          & 64.88                         & 0.58                          & 78.64                         & 1.15                 &       59.99  \\
Linformer~\citep{wang2020linformer} ($k$=256)        & 37.38                         & 0.41                          & 56.12                         & 0.81                          & 79.37                         & 1.62                &        57.62  \\
Performer~\citep{choromanski2020performer} ($r=256$) & 32.78                         & 0.41                          & 65.21                         & 0.82                          & 81.70                         & 1.63                &        59.90  \\
\nformer~\citep{xiong2021nformer} ($l=128$)  & 37.34                         & 0.61                          & 65.75                         & 1.02                          & 81.29                         & 2.03                        &      61.46  \\
\shortname{} ($w,r=8,32$)   & \textbf{37.50}                         & 0.20                         & \textbf{66.01}                         & 0.40                          & 81.79                         & 0.80           &  \textbf{61.77}                \\
\midrule
% Window Attention (best)    & 37.65                         & 0.17                          & \textbf{69.67}                         & 0.28                          & 81.05                         & 0.83      & 62.79                    \\
Dynamic Projection (best)  & 37.79                         & 0.15                          & 66.28                         & 0.69                          & 81.86                         & 2.17           & 61.98               \\
\shortname{} (best)       & \textbf{38.36}                         & 0.16                          & \textbf{68.40}                         & 0.29                          & \textbf{81.95}                         & 2.17   & \textbf{62.90} \\
\bottomrule
\end{tabular}
}
% \vspace{-0.5em}
\end{table}
% End Table %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp!]
\centering
\caption{Comparing the robustness of the models under test-time insertions and deletions. DP refers to long-range attention via Dynamic Projection, and Win. refers to sliding window attention.}
\label{tbl:lra_robust}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lccc|ccc}
\toprule
Task             & \multicolumn{3}{c}{Text}     & \multicolumn{3}{c}{Retrieval} \\
Test Perturb     & None  & Insertion & Deletion & None   & Insertion & Deletion \\
\midrule
Linformer        & 56.12 & 55.94     & 54.91    & 79.37  & 53.66     & 51.75    \\
DP               & 66.28 & 63.16     & 58.95    & 81.86  & \bf{70.01}     & \bf{64.98}    \\
Linformer + Win. & 59.63 & 56.69     & 56.29    & 79.68  & 52.83     & 52.13    \\
DP + Win. (ours) & \bf{68.40}  & \bf{66.34}     & \bf{62.62}    & \bf{81.95}  & 69.93     & 64.19    \\
\bottomrule
\end{tabular}
}
\end{table}
%
\begin{table}[htbp!]
\centering
\setlength{\tabcolsep}{2pt}
% \vspace{-1em}
\caption{Comparing the results of pretrained language models fine-tuned on IMDb.}\label{tbl:imdb}
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Model    & RoBERTa-base & RoBERTa-large & Longformer-base & LS-base             & LS-large \\
\midrule
Accuracy & 95.3         & 96.5          & 95.7            & 96.0                  & \bf{96.8}                 \\
\bottomrule
\end{tabular}
}
% \vspace{-1em}
\end{table}

To evaluate \name{} as a bidirectional encoder for long text, we train our models on the three NLP tasks, \textbf{ListOps}, \textbf{Text}, and \textbf{Retrieval}, from the recently proposed Long Range Arena (LRA) benchmark~\citep{tay2020long}, following the setting of~\citet{peng2021random} and~\citet{tay2021omninet}. For fair comparisons, we use the PyTorch implementation and the same data preprocessing/split, training hyperparameters and model size from \cite{xiong2021nformer}, except for \textbf{Retrieval} where we accidentally used more warmup steps and improved the results for all models. See Appendix~\ref{appendix:lra_configs} for more details. The results on these three tasks are given in Table~\ref{tbl:lra}. Results of the other two image-based tasks of LRA, as well as models implemented in JAX, are given in Appendix~\ref{appendix:lra_additional} and \ref{appendix:lra_jax}. 

In addition, we follow the pretraining procedure of Longformer~\citep{beltagy2020longformer} to pretrain our models based on RoBERTa-base and RoBERTa-large~\citep{liu2019roberta}, and fine-tune it on the IMDb sentiment classification dataset. The results are given in Table~\ref{tbl:imdb}.

%
% Their length statistics are listed in Table~\ref{tbl:lra}.

%
% On all tasks, the models have 2 layers, with embedding dimension $d=64$, head number $h=2$,
% FFN hidden dimension 128, smaller than those from~\citep{tay2020long}. Same as \citep{tay2020long}, we add a CLS token as a global token and use its embedding in the last layer for classification. We re-implement the methods evaluated by~\citet{xiong2021nformer}, and report the best results of our re-implementation and those reported by~\citet{xiong2021nformer}. For our method, we run a grid search on the window size $w$ and the projected dimension $r$, and keep $2w+r\le 256$ to make the complexity similar to the other methods. 
% 

\textbf{Results.}
% 
From Table~\ref{tbl:imdb}, our base model outperforms Longformer-base, and our large model achieves improvements over RoBERTa-large, demonstrating the benefits of learning to model long sequences.
Comparisons with models on LRA are given in Table~\ref{tbl:lra}. 
\shortname{}~(best) with the best configurations of $w,r$ for each task are given in Table~\ref{tbl:lra_configs} in Appendix~\ref{appendix:lra_configs}. We also report the results of using fixed hyperparameter $w=8,r=32$ on all tasks.
Overall, our \shortname{}~(best) is significantly better than other efficient Transformers, and the model with $w,r=8,32$ performs favorably while using only about 50\% to 70\% computation compared to other efficient Transformers on all three tasks. 
The advantage of aggregating local and long-range attentions is the most significant on \textbf{ListOps}, which requires the model to understand the tree structures involving both long-term and short-term relations. 
On \textbf{Retrieval}, where document-level encoding capability is tested, we find our global attention more effective than window attention.
The test accuracy of using only dynamic projection is about 10\% higher than Linformer on \textbf{Text}~(i.e., 66.28 vs. 56.12), which has the highest variance in sequence length~(i.e. standard deviation 893). This demonstrates the improved flexibility of dynamic projection at learning representations for data with high variance in sequence length, compared to the learned but fixed projection of Linformer. 
% 
Similarly, Linformer, \nformer{} and our model outperform full attention on \textbf{ListOps}, indicating they may have better inductive bias, and efficient Transformers can have better efficacy beyond efficiency.

% \subsection{Comparing the robustness against test-time random insertion and deletion}
% \label{appendix:lra_robustness}
\textbf{Robustness of Dynamic Projection. }
In Table~\ref{tbl:lra_robust}, we compare the robustness of Linformer and the proposed Dynamic Projection (DP) against insertion and deletion on Text and Retrieval tasks of LRA. We train the models on the original, clean training sets and only perturb their test sets. For insertion, we insert 10 random punctuations at 10 random locations of each test sample. For deletion, we delete all punctuations from the test samples. Both transforms are label-preserving in most cases. By design, dynamic projection is more robust against location changes.

%

% End of LRA experiments  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% Begin of LM experiments  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-.5em}
\subsection{Autoregressive Language Modeling}
\vspace{-.5em}
%
% 
We compare our method with other efficient transformers on the character-level language modeling where each input token is a character. 

\textbf{Setup.}~ We train and evaluate our model on enwik8 and text8, each with 100M characters and are divided into 90M, 5M, 5M for train, dev, test, following~\citep{Mahoney2009text8}. 
% Throughout training, we set the window size $w=512$, the segment length $l=16$, and the dimension of the dynamic low-rank projection $r=1$, which in our initial experiments achieved better efficiency-accuracy trade-off compared with using $l=32,r=1$ or $l=64,r=4$. 
Our smaller 12-layer and larger 30-layer models are Pre-LN Transformers with the same width and depth as Longformer~\citep{tay2020long}, except that we add relative position encoding to the projected segments in each layer. We adopt the cache mechanism of Transformer-XL~\citep{dai2019transformer}, setting the cache size to be the same as the input sequence length. We follow similar training schedule as Longformer, and train our model in 3 phases with increasing sequence lengths. The input sequence lengths are 2048, 4096 and 8192 respectively for the 3 phases. By comparison, Longformer trains their model in 5 phases on GPUs with 48GB memory (The maximal of ours is 32GB) where the sequence length is 23,040 in the last phase. The window size of Longformer increases with depth and its average window size is 4352 in phase 5, while our effective number of attended tokens is 1280 on average in the last phase.
Each experiment takes around 8 days to finish on 8 V100 GPUs. Detailed hyperparameters are shown in Appendix~\ref{appendix:lm_params}.
%
For testing, same as Longformer, we split the dataset into overlapping sequences of length 32K at a step size of 512, and evaluate the BPCs for predicting the next 512 tokens given the previous 32K characters.

% Begin Figure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
    \includegraphics[width=0.45\textwidth]{figures/autoregressive-mem.pdf}
    \includegraphics[width=0.45\textwidth]{figures/autoregressive-time.pdf}
\end{center}
% \vspace{-1em}
\caption{\footnotesize Running time and memory consumption of Transformer-XL~(full attention) and our \shortname{} on Char-LM. We increase the sequence length until we use up the 32GB of memory on a V100 GPU. \shortname{} is the same smaller model in Table~\ref{tbl:charlm}. We use dashed lines to represent the full attention Transformer and solid lines to represent our model. We use different colors to represent different batch sizes. %\mo{I found the figure legend very confusing. Maybe we explain the legend in the caption?} 
}\label{fig:mem_time}
% \vspace{-1em}
\end{figure}
% End Figure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Results}
%
Table~\ref{tbl:charlm} shows comparisons on text8 and enwik8. Our method has achieved state-of-the-art results. On text8, we achieve a test BPC of 1.09 with the smaller model. On enwik8, our smaller model achieves a test BPC of 0.99, and outperforms the state-of-the-art models with comparable number of parameters. Our larger model obtains a test BPC of 0.97, on par with the Compressive Transformer with 2$\times$ parameters. 
%
Our results are consistently better than Longformer which is trained on longer sequences with 5 stages and 48 GPU memory. 
In Figure~\ref{fig:mem_time}, we show our  model is much more memory and computational efficient than full attention.
% On enwik8, our small model achieves test BPC of 0.987 using just 44M parameters. This is not only significantly better than all current methods with similar model size, but also superior to current methods with over 100M parameters. 
% More ablation studies appear in the appendix. 
% which is great than the results of both 41M small model and 102M large model of Longformer. 

% Begin Table %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\setlength{\columnsep}{10pt}%
\setlength{\tabcolsep}{2pt}
\caption{\footnotesize
BPC ($\downarrow$) of smaller models on enwik8 and text8 (left), and larger models on enwik8 (right). }\label{tbl:charlm}
\vspace{-.2em}
\begin{minipage}{.56\linewidth}
\centering
% \caption{\footnotesize BPC of smaller models on text8/enwik8 test sets.}
 \resizebox{0.9\textwidth}{!}{
 \begin{tabular}{lc|cc|cc}
\toprule
\multirow{2}{*}{Method}   & \multirow{2}{*}{ \#Param}  & \multicolumn{2}{c}{text8} &  \multicolumn{2}{c}{enwik8}\\ 
 &  &  Dev & Test &   Dev & Test  \\ \midrule
 T12~\cite{al2019character} & 44M & -& 1.18 & - & 1.11 \\
 Transformer-XL~\citep{dai2019transformer} & 41M & -  & - & - & 1.06\\
 Reformer~\citep{kitaev2020reformer} & - & -  & - & - & 1.05\\
 Adaptive~\citep{sukhbaatar2019adaptive} & 38M & 1.05 & 1.11 & 1.04 & 1.02 \\ 
BP-Transformer \citep{ye2019bp} & 38M & -  & 1.11 & -  &1.02 \\
Longformer \citep{tay2020long} & 41M &  1.04 & 1.10 & 1.02  &1.00 \\ 
\midrule
\shortname{} & 44M & 1.03 & \textbf{1.09} & 1.01 & \textbf{0.99} \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hspace{.3em}
\begin{minipage}{.43\linewidth}
\centering
% \caption{\footnotesize  BPC of larger models on enwik8 test set.}\label{tbl:charlm}
 \resizebox{0.9\textwidth}{!}{
 \begin{tabular}{lcc}
\toprule
Method                                    & \#Param  &  Test BPC  \\ \midrule
%  T12~\cite{} & 44M & -& 1.18 & - & 1.11 \\
 Transformer-XL~\citep{dai2019transformer} &  88M & 1.03 \\
 Transformer-XL~\citep{dai2019transformer}   & 277M  & 0.99 \\
 Routing~\citep{roy2021efficient}            & 223M & 0.99 \\
 Longformer~\citep{beltagy2020longformer}     & 102M & 0.99 \\
 Sparse~\citep{child2019generating}           &  95M  & 0.99 \\
 Adaptive~\citep{sukhbaatar2019adaptive}      & 209M & 0.98 \\ 
Compressive \citep{rae2019compressive}        & 227M & {\bf 0.97} \\ 
\midrule
\shortname{}                                          & 110M & {\bf 0.97}  \\
\bottomrule
\end{tabular}
}
\end{minipage}
\vspace{-.5em}
\end{table}
% *: results of GPT-2 are zero-shot after trained on the 40GB WebText corpus.
%  GPT-2*~\citep{.radford2019language}  & 117M & - & 1.17 & - & 1.16 \\
%   GPT-2*~\citep{radford2019language}          & 762M & {\bf 0.97} \\
%End Table%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% End of LM experiments  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[]

% \vspace{-.5em}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\centering
\caption{\footnotesize Test accuracies on ImageNet, ImageNet Real~\citep{beyer2020imagenetreal}, and ImageNet V2~\citep{recht2019imagenetv2} of models trained on ImageNet-1K. \textbf{Grey-colored rows are our results}. \cvtname{} denotes our long-short term attention based on the non-official CvT implementation. ViL models with LS suffixes are our long-short term attention based on the official ViL implementation with relative positional bias. We also provide the latency of models tested using batch size 32 on the same V100 GPU. Our improvements over ViL is mainly from a better implementation of the short-term attention.}\label{tbl:image}
\vspace{-.2em}
\setlength{\tabcolsep}{2pt}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|rcrcccc}
\toprule
                                  Model        & \#Param    & Image   & FLOPs     &   ImageNet   & Real       & V2 & Latency\\ 
                                               &  (M)       & Size    &    (G)    &   top-1 (\%) & top-1 (\%) & top-1 (\%) & (s) \\ \midrule \midrule
                                  ResNet-50    & 25          & 224$^2$     & 4.1   & 76.2       & 82.5       & 63.3   & -     \\
                                  ResNet-101   & 45          & 224$^2$     & 7.9   & 77.4       & 83.7      & 65.7    & -    \\
                                  ResNet-152   & 60          & 224$^2$     & 11    & 78.3       & 84.1      & 67.0    & -    \\
\hline
                                DeiT-S~\cite{touvron2020training}    & 22          & 224$^2$        &  4.6   & 79.8   & 85.7    &  68.5  & -       \\
                                DeiT-B~\cite{touvron2020training}    & 86          & 224$^2$        & 17.6   & 81.8   & 86.7    &  70.9  & -        \\
                                \midrule
                                PVT-Medium~\cite{wang2021pyramid}   & 44          & 224$^2$        & 6.7   & 81.2     &  -      &    -   & -       \\
                                PVT-Large~\cite{wang2021pyramid}   & 61          & 224$^2$        & 9.8   & 81.7     &  -      &    -    & -      \\
                                Swin-S~\cite{liu2021swin}          & 50          & 224$^2$        & 8.7   & 83.2     &  -      &    -    & -      \\
                                Swin-B~\cite{liu2021swin}          & 88          & 224$^2$        & 15.4   & 83.5     &  -      &    -   & 0.115       \\
                                PVTv2-B4~\cite{wang2021pvtv2}     & 62.6          & 224$^2$        & 10.1   & 83.6     &  -      &    -  & -        \\
                                PVTv2-B5~\cite{wang2021pvtv2}     & 82.0          & 224$^2$        & 11.8   & 83.8     &  -      &    - & -         \\
                                \midrule
                                ViT-B/16~\citep{dosovitskiy2020image}      & 86          & 384$^2$    & 55.5  & 77.9      &  -      &    -  & -        \\
                                ViT-L/16~\citep{dosovitskiy2020image}      & 307         & 384$^2$    & 191.1 & 76.5       &  -      &    - & -       \\
                                DeiT-B~\citep{touvron2020training}         & 86          & 384$^2$    & 55.5  & 83.1      &  -      &    -  & -       \\
                                Swin-B~\cite{liu2021swin}          & 88          & 384$^2$        & 47.1   & \textbf{84.5}     &  -      &    -  & 0.378        \\
                                \midrule
                                CvT-13~\cite{wu2021cvt}       & 20          & 224$^2$        &  6.7   & 81.6       &  86.7  & 70.4  & 0.122       \\
                                CvT-21~\cite{wu2021cvt}       & 32          & 224$^2$        & 10.1   & 82.5      &  87.2  & 71.3   & 0.165      \\
                                \rowcolor{gray!15}
                                \cvtname{}-13   & 20.3        & 224$^2$        & 4.9   & 81.9          &  87.0 &	70.5 & 0.083 \\
                                \rowcolor{gray!15}
                                \cvtname{}-17   & 23.7        & 224$^2$        & 9.8   & 82.5          & 87.2   &	71.6 & - \\
                                \rowcolor{gray!15}
                                \cvtname{}-21   & 32.1         & 224$^2$        & 7.9   & 82.7     &  87.5      &  71.9 & 0.122 \\
                                \rowcolor{gray!15}
                                \cvtname{}-21S   & 30.1        & 224$^2$        & 11.3   & \textbf{82.9}      & 87.4	& 71.7 & - \\  
                                \midrule
                                CvT-13~\citep{wu2021cvt}          & 20          & 384$^2$        & 31.9   & 83.0      &  87.9  & 71.9  & -        \\
                                CvT-21~\citep{wu2021cvt}          & 32          & 384$^2$        & 45.0   & 83.3      &  87.7  & 71.9  & -       \\
                                \rowcolor{gray!15}
                                \cvtname{}-21   & 32.1       & 384$^2$     & 23.9   & 83.2    &  88.0      &    72.5 & -  \\
                                \rowcolor{gray!15}
                                \cvtname{}-21   & 32.1       & 448$^2$    & 34.2  & \textbf{83.6} & 88.2 &	72.9   & - 	 \\      
                                \midrule
                                ViL-Small~\cite{beltagy2020longformer}    & 24.6        & 224$^2$        & 4.9   & 82.4            &  -      &    -  & -  \\
                                ViL-Medium~\cite{beltagy2020longformer} & 39.7        & 224$^2$        & 8.7   & 83.5            &  -      &    -   & 0.106 \\
                                ViL-Base~\cite{beltagy2020longformer}   & 55.7        & 224$^2$        & 13.4  & 83.7            &  -      &    -   & 0.164 \\
                                \rowcolor{gray!15}
                                ViL-LS-Medium                           & 39.8        & 224$^2$        & 8.7   & 83.8   &  -      &    -    & 0.075  \\
                                \rowcolor{gray!15}
                                ViL-LS-Base                             & 55.8        & 224$^2$        & 13.4   & \textbf{84.1}   &  -      &    -  & 0.113   \\
                                \rowcolor{gray!15}
                                ViL-LS-Medium                           & 39.9        & 384$^2$        & 28.7   & \textbf{84.4}   &  -      &    -  & 0.271    \\
    \bottomrule
\end{tabular}
}
\vspace{-.5em}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{wraptable}{r}{7cm}
% \vspace{-2em}
% \centering
% \caption{\footnotesize Test accuracies of models trained on ImageNet-1K. \textbf{Grey-colored rows are our results}. \cvtname{} denotes our long-short term attention based on the non-official CvT implementation. ViL-\texttt{size}-LS are our models based on the official ViL implementation with relative positional bias. Latencies are tested using batch size 32 on the same V100 GPU. Our improved latency over ViL is mainly from a better implementation of the short-term attention. We give more comparisons in Table~\ref{tbl:image_appendix}.}\label{tbl:image}
% % \vspace{-.2em}
% \setlength{\tabcolsep}{1pt}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{lrcrcccr}
% \toprule
%                                  Model        &  Param    & Image   & FLOPs     &   ImageNet     & Latency\\ 
%                                               &  (M)       & Size    &    (G)    &   top-1 (\%)   & (s) \\ \midrule \midrule
%                                  DeiT-B~\cite{touvron2020training}    & 86          & 224$^2$        & 17.6   & 81.8    & -        \\
%                                  PVT-Large~\cite{wang2021pyramid}   & 61          & 224$^2$        & 9.8   & 81.7       & -      \\
%                                 PVTv2-B5     & 82           & 224$^2$        & 11.8   & 83.8      & -         \\

%                                  Swin-S~\cite{liu2021swin}          & 50          & 224$^2$        & 8.7   & 83.2      & -      \\
%                                  Swin-B~\cite{liu2021swin}          & 88          & 224$^2$        & 15.4   & 83.5     & 0.115       \\
%                                 \midrule
%                                  ViT-B/16~\citep{dosovitskiy2020image}      & 86          & 384$^2$    & 55.5  & 77.9       & -        \\
%                                  ViT-L/16~\citep{dosovitskiy2020image}      & 307         & 384$^2$    & 191.1 & 76.5       & -       \\
%                                  DeiT-B~\citep{touvron2020training}         & 86          & 384$^2$    & 55.5  & 83.1       & -       \\
%                                  Swin-B~\cite{liu2021swin}          & 88          & 384$^2$        & 47.1   & \textbf{84.5}     & 0.378        \\
%                                 \midrule
%                                  CvT-13~\cite{wu2021cvt}       & 20          & 224$^2$        &  6.7   & 81.6      & 0.122       \\
%                                  CvT-21~\cite{wu2021cvt}       & 32          & 224$^2$        & 10.1   & 82.5      & 0.165      \\
%                                 \rowcolor{gray!15}
%                                  \cvtname{}-13   & 20.3        & 224$^2$        & 4.9   & 81.9          & 0.083 \\
%                                 \rowcolor{gray!15}
%                                  \cvtname{}-17   & 23.7        & 224$^2$        & 9.8   & 82.5          & - \\
%                                 \rowcolor{gray!15}
%                                  \cvtname{}-21   & 32.1         & 224$^2$        & 7.9   & 82.7     &   0.122 \\
%                                 \rowcolor{gray!15}
%                                  \cvtname{}-21S   & 30.1        & 224$^2$        & 11.3   & \textbf{82.9}      & - \\  
%                                 \midrule
%                                  CvT-13~\citep{wu2021cvt}          & 20          & 384$^2$        & 31.9   & 83.0     & -        \\
%                                 CvT-21~\citep{wu2021cvt}          & 32          & 384$^2$        & 45.0   & 83.3      & -       \\
%                                 \rowcolor{gray!15}
%                                 \cvtname{}-21   & 32.1       & 384$^2$     & 23.9   & 83.2    & -  \\
%                                 \rowcolor{gray!15}
%                                 \cvtname{}-21   & 32.1       & 448$^2$    & 34.2  & \textbf{83.6} & - 	 \\      
%                                 \midrule
%                                 ViL-S~\cite{beltagy2020longformer}    & 24.6        & 224$^2$        & 4.9   & 82.4           & -  \\
%                                 ViL-M   & 39.7        & 224$^2$        & 8.7   & 83.5            & 0.106 \\
%                                 ViL-B~\cite{beltagy2020longformer}   & 55.7        & 224$^2$        & 13.4  & 83.7            & 0.164 \\
%                                 \rowcolor{gray!15}
%                                 ViL-LS-M                           & 39.8        & 224$^2$        & 8.7   & 83.8    & 0.075  \\
%                                 \rowcolor{gray!15}
%                                 ViL-LS-B                             & 55.8        & 224$^2$        & 13.4   & \textbf{84.1}    & 0.113   \\
%                                 \rowcolor{gray!15}
%                                 ViL-LS-M                           & 39.9        & 384$^2$        & 28.7   & \textbf{84.4}    & 0.271    \\
%     \bottomrule
% \end{tabular}
% }
% \end{wraptable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-.5em}
\subsection{ImageNet Classification}
\vspace{-.5em}
We train and evaluate the models on ImageNet-1K with 1.3M images and 1K classes.
%
We use CvT~\citep{wu2021cvt} and ViL~\citep{zhang2021visionlongformer}, state-of-the art vision transformer architectures, as the backbones and replace their  attention mechanisms with our long-short term attention, denoted as \cvtname{} and ViL-\texttt{size}-LS in Table~\ref{tbl:image}. 
CvT uses overlapping convolutions to extract dense patch embeddings from the input images and feature maps, resulting in a long sequence length in the early stages~(e.g., $56\times56 = 3136$ patches for images with $224^2$ pixels).
For ViL, our sliding window uses the same group size $w$, but each token attends to at most $2w\times 2w$ (rounding when necessary) tokens inside the window, instead of $3w\times 3w$ as ViL, which allows adding our dynamic projection without increasing the FLOPs. We set $r=8$ for the dynamic projections for both ViL-LS-Medium and ViL-LS-Base.
Note that, our efficient attention mechanism does not depend on the particular architecture, and it can be applied to other vision transformers~\citep[e.g.,][]{dosovitskiy2020image,touvron2020training,wang2021pyramid}. 
Please refer to Appendix~\ref{appendix:image_params} for more details.

 
\textbf{Classification Results.}
The results are shown in the Table~\ref{tbl:image}, where we also list test accuracies on ImageNet Real and ImageNet V2. Except for CvT, we compare with the original ViT~\citep{dosovitskiy2020image} and the enhanced DeiT~\citep{touvron2020training}, PVT~\citep{wang2021pyramid} that also uses multi-scale stragey, 
ViL~\citep{zhang2021visionlongformer} that uses window attention and global tokens to improve the efficiency. 
%
%
Training at high-resolution usually improves the test accuracy of vision transformer. With our long-short term attention, we can easily scale the training to higher resolution, and the performance of \cvtname{} and ViL-LS also improves. Our best model with CvT~(\cvtname{}-21 at $448^2$) achieves 0.3\% higher accuracy than the best reported result of CvT while using the same amount of parameters and 76\% of its FLOPs.
In CvT architecture, the spatial dimension of feature maps in earlier stages are large, representing more fine-grained details of the image. Similar to training with high-resolution images, the model should also benefit from denser feature maps. With our efficient long-short term attention, we can better utilize these fine-grained feature maps with less concerns about the computational budget. In this way, our \cvtname{}-17 achieves better result than CvT-21 at resolution 224 using fewer parameters and FLOPs, and our \cvtname{}-21S model further improves our \cvtname{}-21 model.

Our ViL-LS-Medium and ViL-LS-Base with long-short term attention improve the accuracies of ViL-Medium and ViL-Base from 83.5 and 83.7 to 83.8 and 84.1 respectively, without an increase in FLOPs. When increasing the resolution for training ViL-LS-Medium from $224^2$ to $384^2$, the FLOPs increased (approximately) linearly and the accuracy improved by 0.6\%, showing our method still benefits greatly from increased resolution while maintaining the linear complexity in practice.



\textbf{Short-term Attention Suppresses Oversmoothing.}
By restricting tokens from different segments to attend to different windows, our short-term sparse local attention encourages diversity of the feature representations and helps to alleviate the over-smoothing problem~\citep{gong2021improve} (where all queries extract similar information in deeper layers and the attention mechanism is less important), thus can fully utilize the depth of the network. As in \citep{gong2021improve}, we provide the cosine similarity of patch embeddings of our \cvtname{}-13 and re-implemented CvT-13 (81.1 accuracy) in Figure~\ref{fig:cos_sim} within Appendix. This is one of the reasons why our efficient attention mechanism can get even better results than the full attention CvT model in the same setting.


%% Table: latency comparisons
% \begin{table}[htbp!]
% \setlength{\tabcolsep}{2pt}
% \centering
% \caption{Comparing the latency of models trained on ImageNet-1k.}
% \begin{tabular}{lccrrc}
% \toprule
% Model         & Res. & Top-1 (\%) & Params & FLOPs & Latency  \\
% \midrule
% Swin-B        &  $224^2$   & 83.3       & 88M            & 15.4G      & 0.115s       \\
% Swin-B        &  $224^2$   & 84.5       & 88M            & 47G        & 0.378s       \\
% ViL-Medium    &  $224^2$   & 83.5       & 39.7M          & 8.7G      & 0.106s       \\
% ViL-Base      &  $224^2$   & 83.7       & 55.7M          & 13.4G      & 0.164s       \\
% \midrule
% ViL-LS-Medium &  $224^2$   & 83.8       & 39.8M          & 8.7G       & 0.075s       \\
% ViL-LS-Base   &  $224^2$   & 84.1       & 55.8M          & 13.4G      & 0.113s       \\
% ViL-LS-Medium &  $384^2$   & 84.4       & 39.8M          & 28.7G      & 0.271s      \\
% \bottomrule
% \end{tabular}
% \end{table}
%%

 
\textbf{Robustness evaluation on Diverse ImageNet Datasets.}
%
% Begin of robustness results%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
% \vspace{-1em}
\setlength{\tabcolsep}{2pt}
\centering
\caption{\footnotesize Robustness evaluation on various ImageNet datasets. Top-1/Acc.: Top-1 accuracy. mCE: Mean Corrupution Error. Mixed-same/Mixed-rand: accuracies on \textsc{Mixed-Same}/\textsc{Mixed-Rand} subsets. }\label{tbl:robustness}
\vspace{-.3em}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|cc}
\toprule
Model                                  & Params & ImageNet    & IN-C~\citep{hendrycks2018imagenetc} &  IN-A~\cite{hendrycks2019natural} & IN-R~\cite{hendrycks2020many} & \multicolumn{2}{c}{ImageNet-9~\cite{xiao2020noise}}   \\
\midrule
                                       & (M)    & Top-1       & mCE ($\downarrow$) & Acc. & Acc. & Mixed-same & Mixed-rand  \\
\midrule
ResNet-50~\citep{he2016deep}           & 25.6   & 76.2  & 78.9               & 6.2  & 35.3 & 87.1       & 81.6        \\
DeiT-S~\citep{touvron2020training}     & 22.1   & 79.8  & 57.1               & 19.0 & 41.9 & 89.1       & 84.2        \\
CvT-13	                               & 20     & 81.6	& 59.6	& 25.4	& 42.9	& 90.5	& 85.7 \\
CvT-21	                               & 32     & 82.5	& 56.2	& \textbf{31.1}	& 42.6	& 90.5	& 85.0 \\
\cvtname{}-13                          & 20.3   & 81.9  & 58.7               & 27.0 & 42.6 & 90.7       & 85.6        \\
\cvtname{}-21                          & 32.1   & \textbf{82.7}  & \textbf{55.2} & {29.3} & \textbf{45.0} & \textbf{91.5} & \textbf{85.8}        \\
\bottomrule
\end{tabular}
}
\vspace{-1em}
\end{table}
% End of robustness results%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As vision models have been widely used in safety-critical applications (e.g. autonomous driving), their robustness is vital.  
In addition to out-of-distribution robustness (ImageNet-Real and Imageet-v2), we further investigate the robustness of our vision transformer against  common corruption (ImageNet-C), semantic shifts (ImageNet-R), Background dependence (ImageNet-9) and natural adversarial examples (ImageNet-A). We compare our methods with standard classification methods, including CNN-based model  (ResNet~\cite{he2016deep}) and Transformer-based models (DeiT~\cite{touvron2020training}) with similar numbers of parameters. 
As shown in Table~\ref{tbl:robustness}, we observe that our method significantly outperforms the CNN-based method (ResNet-50).
% Such results further empirically verify the importance of attention mechanisms for the robustness of vision models. 
Compared to DeiT, our models also achieve favorable improvements. These results indicate that the design of different attention mechanisms plays an important role for model robustness, which sheds new light on the design of robust vision transformers.
More details and results can be found in Appendix~\ref{appendix:image_params}.





==> Long-Short Transformer - NeurIPS 2021/sections/method.tex <==


\vspace{-.3em}
\section{Long-Short Transformer}
\label{sec:method}
\vspace{-.2em}
%

\begin{figure}
\begin{center}
\includegraphics[width=\textwidth]{figures/general_framework.pdf}
\end{center}
\vspace{-1em}
\caption{\footnotesize
Long-short term attention of a single attention head. Here, the sequence length $n=8$, hidden dimension $d=3$, local window segment size $w=2$, and rank of dynamic projection $r=3$. 
Within the figure, $K(V)$ denotes key $K$ or value $V$.
In the left figure, we virtually replicate $K$ or $V \in \sR^{n\times d}$ into $n$ rows, and highlight the keys and values within the attention span (denoted as $\tilde{K} (\tilde{V})$) of all $n$ queries $Q$ for the short-term attention. In the middle figure, all queries attend to the same projected keys $\bar{K}$ and values $\bar{V}$ within the long-term attention. In the right figure, $\tilde{K}(\tilde{V})$ and $\bar{K}(\bar{V})$ are first normalized with two sets of LayerNorms, and the queries attend to normalized $\tilde{K}(\tilde{V})$ and $\bar{K}(\bar{V})$ within their attention span simultaneously.}
\label{fig:general}
% \vspace{-1em}
\end{figure}

\shortname{} approximates the full attention by aggregating long-range and short-term attentions, while maintaining its ability to capture correlations between all input tokens.
In this section, we first introduce the preliminaries of multi-head attention in Transformer.
Then, we present the short-term attention via sliding window, and long-range attention via dynamic projection, respectively.
After that, we propose the aggregating method and dual normalization~(DualLN) strategy. See Figure~\ref{fig:general} for an illustration of our long-short term attention.


\subsection{Preliminaries and Notations}
%
Multi-head attention is a core component of the Transformer~\citep{vaswani2017attention}, which computes contextual representations for each token by attending to the whole input sequence at different representation subspaces. It is defined as
\begin{equation}
    \multihead{}(Q,K,V)=\text{Concat}(H_1,H_2,...,H_h)W^O,
\end{equation}
where $Q, K, V \in \sR^{n\times d}$ are the query, key and value embeddings, $ W^O\in \sR^{d\times d}$ is the projection matrix for output, the $i$-th head $H_i \in \sR^{n\times d_k}$ is the scaled dot-product attention, and $d_k=d/h$ is the embedding dimension of each head,
\begin{equation}
    H_i=\attention{}(QW_i^{Q}, KW_{i}^K, VW_{i}^V)=\softmax{}\left[\frac{QW_i^{Q} \left( KW_{i}^K \right)^\intercal }{\sqrt{d_k}}\right]VW_i^V=A_i VW_i^V,
\end{equation}
where $W_i^Q,W_i^K,W_i^V\in \sR^{d\times d_k}$ are learned projection matrices, and $A_i\in \sR^{n\times n}$ denotes the full attention matrix for each attention head. The complexity of computing and storing $A_i$ is  $O(n^2)$, which can be prohibitive when $n$ is large.
For simplicity, our discussion below is based on the case of 1D input sequences. It is straightforward to extend to the 2D image data given a predetermined order. 


\vspace{-.2em}
\subsection{Short-term Attention via Segment-wise Sliding Window}
\vspace{-.2em}
%
We use the simple yet effective sliding window attention to capture fine-grained local correlations, where each query attends to nearby tokens within a fixed-size neighborhood.
%
Similar techniques have also been adopted in~\citep{beltagy2020longformer,zaheer2020big, zhang2021visionlongformer}. Specifically, we divide the input sequence into disjoint segments with length $w$ for efficiency reason. All tokens within a segment attend to all tokens within its home segment, as well as $w/2$ consecutive tokens on the left and right side of its home segment (zero-padding when necessary), resulting in an attention span over a total of $2w$ key-value pairs. See Figure~\ref{fig:window_attention} in Appendix for an illustration.
%
For each query $Q_t$ at the position $t$ within the $i$-th head, we denote the $2w$ key-value pairs within its window as $\tilde{K}_{t},\tilde{V}_t \in \sR^{2w\times d}$. For implementation with PyTorch, this segment-wise sliding window attention is faster than the per-token sliding window attention where each token attends to itself and $w$ tokens to its left and right, and its memory consumption scales linearly {with sequence length}; see~\citep{beltagy2020longformer} and our Figure~\ref{fig:mem_time} for more details. 

The sliding window attention can be augmented to capture long-range correlations in part, by introducing different dilations to different heads of sliding window attention~\citep{beltagy2020longformer}. However, the dilation configurations for different heads need further tuning and an efficient implementation of multi-head attention with different dilations is non-trivial. A more efficient alternative is to augment sliding window attention with random sparse attention~\citep{zaheer2020big}, but this does not guarantee that the long-range correlations are captured in each layer as in full attention. 
In the following section, we propose our long-range attention to address this issue.



\vspace{-.2em}
\subsection{Long-range Attention via Dynamic Projections}
\label{sec:low_rank}
\vspace{-.2em}
Previous works have shown that the self-attention matrix can be well approximated by the product of low-rank matrices~\citep{wang2020linformer}.
% 
By replacing the full attention with the product of low-rank matrices~\citep{katharopoulos2020lineartrans,tay2020synthesizer,xiong2021nformer,peng2021rfa,choromanski2020performer}, each query is able to attend to all tokens. 
Linformer~\citep{wang2020linformer} is one of the most representative models in this category. It learns a fixed projection matrix to reduce the length of the keys and values, but the fixed projection is inflexible to semantic-preserving positional variations.

Starting from these observations, we parameterize the dynamic low-rank projection at $i$-th head as $P_i = f(K) \in \sR^{n\times r}$, where $r \ll n$ is the low rank size and $P_i$ depends on all the keys $K \in \sR^{n\times d}$ of input sequence.
It projects the $(n\times d_k)$-dimensional key embeddings $KW_i^K$ and value embeddings $VW_i^V$ into shorter, $(r\times d_k)$-dimensional key $\bar{K}_i$ and value $\bar{V}_i$ embeddings.
%
Unlike Linformer~\citep{wang2020linformer}, the low-rank projection matrix is dynamic, which depends on the input sequence and is intended to be more flexible and robust to, e.g., insertion, deletion, paraphrasing, and other operations that change sequence length. See Table~\ref{tbl:lra_robust} for examples.
%
Note that, the query embeddings $QW_i^Q \in \sR^{n\times d_k}$ are kept at the same length, and we let each query attend to $\bar{K}_i$ and $\bar{V}_i$. 
In this way, the full $(n\times n)$ attention matrix can be decomposed into the product of two matrices with $r$ columns or rows.
Specifically, we define the dynamic projection matrix $P_i \in \sR^{n\times r}$ and the key-value embeddings $\bar{K}_i,\bar{V}_i \in \sR^{r\times d_k}$ of low-rank attention as 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\label{eq:dmem}
P_i = \softmax{}(KW_i^P),~ \bar{K}_i=P_i^\intercal  KW_i^K, \bar{V}_i=P_i^\intercal  VW_i^V,
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $W_i^P\in \sR^{d\times r}$ are learnable parameters,\footnote{For the CvT-based vision transformer model, we replace $W_i^P$ with a depth-wise separable convolution, just as its query, key and value projections.} 
and the softmax normalizes the projection weights on the first dimension over all $n$ tokens, which stabilizes training in our experiments. Note that $K=V$ in all the experiments we have considered, so $P_i$ remains the same if it depends on $V$. 
The computational complexity of Eq.~\ref{eq:dmem} is $O(rn)$.
% \zc{TODO: justify the choice of softmax, instead of unbounded weights like Linformer.}

To see how the full attention is replaced by the product of low-rank matrices, we compute each head $H_i \in \sR^{n\times d_k}$ of long-range attention as,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
    \bar{H}_i = \underbrace{\softmax{}\left[\frac{QW_i^Q \bar{K}_i^\intercal }{\sqrt{d_k}}\right]}_{\bar{A}_i}\bar{V}_i =\bar{A}_i \big( P_i^\intercal VW_i^V \big),
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
so the full attention is now replaced with the implicit product of two low-rank matrices $\bar{A}_i\in \sR^{n\times r}$ and $P_i^\intercal\in \sR^{r\times n}$, and the computational complexity is reduced to $O(rn)$. 
Note the effective attention weights of a query on all tokens still sum to 1.  Our global attention allows each query to attend to all token embeddings within the same self-attention layer.
In contrast, the sparse attention mechanisms~\citep{beltagy2020longformer, zaheer2020big} need stack multiple layers to build such correlations.



\textbf{Application to Autoregressive Models:}~ 
In autoregressive models, each token can only attend to the previous tokens, so the long-range attention should have a different range for different tokens. A straightforward way to implement our global attention is to update $\bar{K}_i,\bar{V}_i$ for each query recurrently, but this requires re-computing the projection in Eq.~\eqref{eq:dmem} for every token due to the nonlinearity of softmax, which results in $O(rn^2)$ computational complexity. To preserve the linear complexity, for autoregressive models, we first divide the input sequence into equal-length segments with length $l$, and apply our dynamic projection to extract $\bar{K}_{i},\bar{V}_{i}$ from each segment. Each token can only attend to $\bar{K}_i,\bar{V}_i$ of segments that do not contain its future tokens. Formally, let $Q_t$ be the query at position $t$, $K_{(l-1)s:ls},V_{(l-1)s:ls}$ be the key-value pairs from the $s$-th segment, and $s_t=\lfloor{t/l}\rfloor$. For autoregressive models, we compute the long-range attention of $Q_t$ by attending to $K_{i,t},V_{i,t}$, defined as
\begin{equation}
  \bar{K}_{i,t} =  [P_{i,1}^\intercal K_{1:l};...;P_{i,s_t}^\intercal K_{(l-1)s_t:ls_t}]W_i^K,
  \bar{V}_{i,t} =  [P_{i,1}^\intercal V_{1:l};...;P_{i,s_t}^\intercal V_{(l-1)s_t:ls_t}]W_i^V.
\end{equation}
In this way, the dynamic low-rank projection is applied to each segment only once in parallel, preserving the linear complexity and the high training speed. By comparison, Random Feature Attention~\citep{peng2021random} is slow at training due to the requirement for recurrence.

% End of subsection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Aggregating Long-range and Short-term Attentions}
%
To aggregate the local and long-range attentions, instead of adopting different attention mechanisms for different heads~\citep{child2019generating,beltagy2020longformer,wu2020lite}, we let each query at $i$-th head attend to the union of keys and values from the local window and global low-rank projections, thus it can learn to select important information from either of them.
We find this aggregation strategy works better than separating the heads in our initial trials with the autoregressive language models. 
Specifically, for the $i$-th head, we denote the global low-rank projected keys and values as $\bar{K}_i,\bar{V}_i \in \sR^{r\times d_k}$,
and the local keys and values as $\tilde{K}_t,\tilde{V}_t \in \sR^{2w\times d}$ within the local window of position $t$ for the query $Q_t$. 
Then the $i$-th attention $H_{i, t}$ at position $t$ is
\begin{equation}
     {H}_{i,t} = \softmax{}\left[\frac{Q_t W_i^Q\left[\tilde{K}_t W_i^K; \bar{K}_i\right]^\intercal }{\sqrt{d_k}}\right] [\tilde{V}_t W_i^V;\bar{V}_i].
\end{equation}
where $[\cdot~;\cdot]$ denotes concatenating the matrices along the first dimension.
Furthermore, we find a scale mismatch between the initial norms of $\tilde{K}_tW_i^K$ and $\bar{K}_i$, which biases the attention to the local window at initialization for both language and vision tasks. We introduce a normalization strategy~(DualLN) to align the norms and improve the effectiveness of the aggregation in the following.



% Begin of subsection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.55\textwidth]{figures/init-norm-ratios.pdf}
% \includegraphics[width=0.55\textwidth]{figures/autoregressive-norm-ratios.pdf}
\includegraphics[width=0.4\textwidth]{figures/dualln_charlm.pdf}
\end{center}
% \vspace{-1em}
\caption{\footnotesize
Left: Ratios of the average $\ell_2$ norms of the local window to global low-rank key/value embeddings at initialization. Without DualLN, the sparse and low-rank embeddings have a magnitude mismatch. With DualLN, the ratios will be $1.0$ at every layer, which will facilitate optimization.  
Right: The validation loss of \shortname{} with and without DualLN on enwik8 and text8.}
\label{fig:lmln}
% \vspace{-1em}
\end{figure}

\textbf{DualLN:} 
For Transformers with Layer Normalization~(LN)~(see \citep{xiong2020layer} for an illustration), the $K_i,V_i$ embeddings are the outputs of LN layers, so they have zero mean and unit variance at initialization. The $\ell_2$ norm of vectors with zero-mean entries is proportional to their variance in expectation. 
We note a weighted average will reduce the variance and therefore the norm of such zero-mean vectors. 
As a result, the embedding vectors from low-rank attention in the weighted average $\bar{K}_i,\bar{V}_i$ of Eq.~\eqref{eq:dmem} will have smaller norms than the regular key and value embeddings from sliding window attention~(see Figure~\ref{fig:lmln} Left for an illustration).
%
This scale mismatch causes two side effects. First, the inner product $Q_t W_i^Q \bar{K}_i^\intercal $ from local-rank component tends to have smaller magnitude than the local window one, thus the attention scores on long-range attention is systematically smaller. 
Second, the key-value pairs $\bar{K}_i,\bar{V}_i$ for the low-rank attention will naturally have less impact on the direction of $H_i$ even when low-rank and local window are assigned with same attention scores, since $\bar{V}_i$ has smaller norms. 
Both effects lead to small gradients on the low-rank components and hinders the model from learning to effectively use the long-range correlations.

To avoid such issues, we add two sets of Layer Normalizations after the key and value projections for the local window and global low-rank attentions, so that their scales are aligned at initialization, but the network can still learn to re-weight the norms after training. Specifically, the aggregated attention is now computed as
\begin{equation}\label{eq:attn_final}
     {H}_{i,t} = \softmax{}\left[\frac{Q_t W_i^Q\left[\layernorm{}_L(\tilde{K}_t W_i^K); \layernorm{}_G(\bar{K}_i)\right]^\intercal }{\sqrt{d_k}}\right] [\layernorm{}_L(\tilde{V}_t W_i^V); \layernorm{}_G(\bar{V}_i)],
\end{equation}
where $\layernorm{}_L(\cdot), \layernorm{}_G(\cdot)$ denote the Layer Normalizations for the local and global attentions respectively. 
In practice, to maintain the consistency between the local attention and dynamic projection, we use $\text{LN}_{L}(K),\text{LN}_{L}(V)$ instead of $K,V$ to compute $\bar{K}_i,\bar{V}_i$ in Eq.~\ref{eq:dmem}.
As illustrated in Figure~\ref{fig:lmln} Right, the \shortname{} models trained with DualLN has consistently lower validation loss than the models without DualLN.

% End of subsection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work? 
    \answerYes{} We mentioned that as our future work in the conclusion section.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} Yes, we have included an investigation into the robustness of our vision models in the experiments. Also see Broader Impacts Section in Appendix.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
